Achieving Socio-Economic Parity through the Lens of EU AI Act

Unfair treatment and discrimination are critical ethical concerns in AI systems, particularly as their adoption expands across diverse domains. Addressing these challenges, the recent introduction of the EU AI Act establishes a unified legal framework to ensure legal certainty for AI innovation and investment while safeguarding public interests, such as health, safety, fundamental rights, democracy, and the rule of law (Recital 8). The Act encourages stakeholders to initiate dialogue on existing AI fairness notions to address discriminatory outcomes of AI systems. However, these notions often overlook the critical role of Socio-Economic Status (SES), inadvertently perpetuating biases that favour the economically advantaged. This is concerning, given that principles of equalization advocate for equalizing resources or opportunities to mitigate disadvantages beyond an individual's control. While provisions for discrimination are laid down in the AI Act, specialized directions should be broadened, particularly in addressing economic disparities perpetuated by AI systems. In this work, we explore the limitations of popular AI fairness notions using a real-world dataset (Adult), highlighting their inability to address SES-driven disparities. To fill this gap, we propose a novel fairness notion, Socio-Economic Parity (SEP), which incorporates SES and promotes positive actions for underprivileged groups while accounting for factors within an individual's control, such as working hours, which can serve as a proxy for effort. We define a corresponding fairness measure and optimize a model constrained by SEP to demonstrate practical utility. Our results show the effectiveness of SEP in mitigating SES-driven biases. By analyzing the AI Act alongside our method, we lay a foundation for aligning AI fairness with SES factors while ensuring legal compliance.

==> stavroula_intro+sociological_pespective.tex <==
Bias, which derives from AI systems, can result in unfair treatment and discrimination \cite{hleg2019ethics, information_commissioners_office_ico_guidance_2024} and has been recognised as a major ethical concern for AI systems \cite{access_now_human_2018, latonero_governing_2018, muller_impact_2020}.
More specifically, AI bias constitutes the “systematic and repeatable errors in a computer system that create unfair outcomes, such as favoring one arbitrary group of users over others”; fairness in the context of AI systems is established by preventing unfair bias, discrimination and stigmatisation \cite{hleg2019ethics,ala2020assessment}. In this paper, the term "AI fairness" refers to the risk of discrimination arising from algorithmic or AI bias, in accordance with the extensive literature in the field of fairness metrics in machine learning. While several AI fairness metrics have emerged in the field of machine learning (for an overview: \cite{barocas_fairmlbook,castelnovo2022clarification}), an important layer to be examined is their interference and possible integration with the newly enacted  European Union (EU) AI Act \cite{noauthor_regulation_2024}. On one hand, the determination and implementation of fairness metrics for AI bias must take into account the applicable legal framework, while on the other hand, the fairness metrics utilised in machine learning have the potential to initiate discussions regarding new standards\footnote{On May 22, 2023, the European Commission (EC) issued a standardisation request to CEN and the CENELEC regarding AI Act (Implementing decision C(2023)3215). Available at: https://ec.europa.eu/growth/tools-databases/enorm/mandate/593\_en.}, guidelines and assessment tools as they are able to provide practical solutions. 
\par A unified legal framework for AI, promotes legal certainty to promote innovation and investment in AI \cite{din2020german}, while ensuring strong safeguards for public interests such as health, safety, fundamental rights, democracy, the rule of law as mandated by EU law (Recital 8, AI Act). The specialised AI legislation in the EU environment is governed by the AI Act, which is one of the first bidding legal instruments and the most comprehensive and strictest worldwide. Its scope, which targets also providers that place AI systems or placing on the market general-purpose AI models into EU “…\textit{irrespective of whether those providers are established or located},” determines the global effect of the AI Act, as also non-EU based entities and individuals, will have to comply with it, under the circumstances of Article 2, thus demonstrating the extra-territorial scope of the AI Act \cite{greenleaf2021brussels}. Several countries introduced relevant legislation after the proposal of the AI Act in 2021 and can be considered part of the Brussels effect \cite{bradford2020brussels}. Notably, on the other side of the Atlantic, the USA issued the \textit{Executive Order on Safe, Secure, and Trustworthy Artificial Intelligence} in October 2023 \footnote{Exec. Order No. 14110, 88 FR 75191, pp. 75191-75226 (October 30, 2023). Available at: https://www.whitehouse.gov/briefing-room/statements-releases/2023/10/30/
fact-sheet-president-biden-issues-executive-order-on-safe-secure-and-trustworthy-artificial-intelligence.
}.  The continuously increasing trend in the global adoption of laws related to artificial intelligence has become evident in recent years \cite{etchemendy_ai_2024}, while the proposal of the AI Act in 2021 led to a 1.200\% increase\footnote{This calculation was made based on the public data for the years 2021 and 2022, from the AI Index 2024 Annual Report by Stanford University \cite{ai_index_steering_committee_institute_for_human-centered_ai_stanford_university_ai_nodate}.} (in the year following the proposal, namely 2022), further strengthening the belief in its global influence along with the increasing influence of AI across all aspects of society. Undoubtedly, the AI fairness field of machine learning demands a means of standardisation in terms of the up-to-date applicable legal requirements. And as has been widely argued, it is not the pursuit of a universal solution \cite{deck2024implications, information_commissioners_office_ico_guidance_2024, wachter2021fairness} for determining the appropriate fairness metric, but rather the identification of ad hoc solutions that is essential. Therefore, drawing upon socioeconomic status (SES), which has been asserted to necessitate increased attention due to its legal protection in relation to discrimination grounds \cite{ganty2021expanding}, as well as its possible implications through the lens of AI applications. In this paper, we examine the SES case, with the purpose of generalising the proposed solutions and integration in the AI Act requirements for AI bias. The importance of tackling the feedback loop of socio-economic precariousness has been recognised \cite{ganty2021poverty}, as well as the potential consideration by the courts of vulnerable groups, characterised by SES due to structural disadvantages \cite{gerards2022protected}. Despite a growing body of research highlighting the prevalence of discrimination based on SES and the urgent need to address it \cite{atrey2018intersectional,kadar2016analysis,benn2020big,ganty2021expanding,niall_crowley_equality_2015}, this factor has not yet been fully integrated into the anti-discrimination EU legal frameworks \cite{ganty2021expanding}. Through the adoption of the AI Act, the investigation of this important context can be rendered more effective, as fairness metrics may be anchored in established standards. Furthermore, it can stimulate discussions regarding the legal management of AI bias that adversely affects SES. While this paper examines the realisation of predictive fairness within the socioeconomic context, as interpreted through the framework of the AI Act, the conceptual solutions and recommendations may prove beneficial for scholars and in other regions, not only due to the extraterritoriality of the AI Act, which has been discussed above in this Section, but also because of similar challenges related to the efficiency of the AI fairness metrics in relation to the legal requirements.

\subsubsection{\textbf{Extraction supported by contextual data from a sociological perspective}}\todo[author=Stavroula]{We can also transfer this subsection to the next steps}
Apart from the legal dimensions of the automated identification of the features, it should be argued that their investigation can be further supported by statistical data and relevant socio-economic studies focused on the specific context. This evidence should pertain to a geographically defined population group and rely on an extended approach that aligns with the capacity to strengthen arguments for the existence of discrimination and its interference with specific group features, such as the CJEU may accept statistical evidence, as previously mentioned. Notably, in the context of SES, it has been argued that ``occupation'' serves as an indicator of an individual's position and facilitates the classification of individuals based on their SES \cite{csatho2023broken}. At the EU level, the gender gap via statistical evidence, which is a discriminatory dimension of the SES, between men and women has revealed that the following factors are crucial in displaying inequalities: sector of occupation, work hours per week, the hierarchical position of the occupation, equal pay \cite{eu_gender_pay_gap}. From a sociological perspective, one should also consider the contribution of co-creation processes, involving stakeholders and training, in the process of identifying the characteristics that AI fairness solutions should encompass \cite{slesinger2024training}.

==> temporary.tex <==
%%%%%%current version
Unfair treatment and discrimination \cite{hleg2019ethics, information_commissioners_office_ico_guidance_2024}—commonly referred to as AI bias or unfairness—are widely recognized as significant ethical concerns in AI systems \cite{access_now_human_2018, latonero_governing_2018, muller_impact_2020}. The pervasive integration of AI across various societal and economic domains has amplified the urgency of addressing these issues. This is further underscored by the increasing global adoption of AI-related legal frameworks \cite{etchemendy_ai_2024}, including the landmark EU AI Act proposed in 2021, which catalyzed a 1,200\% increase\footnote{Based on public data for 2021 and 2022 from the AI Index 2024 Annual Report by Stanford University \cite{ai_index_steering_committee_institute_for_human-centered_ai_stanford_university_ai_nodate}.} in regulatory activities in the following year. While the Act provides a comprehensive framework for addressing discrimination, its scope should be broadened to include specialized directions targeting economic disparities perpetuated by AI systems~\cite{ganty2021expanding}.

These disparities are deeply rooted in socio-economic status (SES), which disproportionately affects historically marginalized groups~\cite{ganty2021expanding}. For instance, individuals subjected to discrimination based on traditional status grounds, such as gender and race, are often overrepresented among economically disadvantaged populations~\cite{ganty2021poverty}. This intersectionality of SES with existing vulnerabilities exacerbates systemic inequities~\cite{atrey2018intersectional}, violating principles of equalization~\cite{dworkin2018equality}, which advocate for equalizing resources or opportunities to mitigate disadvantages beyond an individual's control.

Despite advancements in AI fairness metrics \cite{barocas_fairmlbook, castelnovo2022clarification}, most fail to capture the compounded effects of economic privilege. This creates critical gaps in addressing SES-driven disparities that produce unfair advantages across protected features like gender~\cite{kilbourne1997ses_gender} and race~\cite{williams2017wealth,kochhar2014wealth}.

To address this gap, we propose a novel fairness notion, Socio-Economic Parity (SEP), and its stricter variant, Conditional Socio-Economic Parity (CSEP). These notions explicitly incorporate SES into fairness considerations, emphasizing positive actions for underprivileged groups while accounting for individual-level factors such as working hours. Using a real-world dataset (Adult~\cite{adult}), we demonstrate that existing fairness notions—such as Equal Opportunity~\cite{hardt2016equality}, Demographic Parity~\cite{dwork2012fairness}, and Conditional Demographic Parity (CDP)~\cite{toon2012book}—fail to address SES-driven disparities and inadvertently reinforce biases favouring economically privileged groups.

Our empirical results highlight the effectiveness of SEP and CSEP in measuring and mitigating SES-driven bias. Furthermore, through an analytical study of the AI Act in parallel with our proposed methods, we establish a foundation for fostering dialogues that align AI fairness with economic and financial applications. This work bridges the gap between fairness-aware machine learning research and regulatory frameworks, emphasizing the importance of addressing socio-economic disparities in AI systems.



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Unfair treatment and discrimination \cite{hleg2019ethics, information_commissioners_office_ico_guidance_2024}—commonly referred to as AI bias or unfairness—are widely recognized as significant ethical concerns in AI systems \cite{access_now_human_2018, latonero_governing_2018, muller_impact_2020}. The pervasive integration of AI across various societal and economic domains has amplified the need to address these issues. This urgency is underscored by the increasing global adoption of AI-related legal frameworks \cite{etchemendy_ai_2024}, including the landmark EU AI Act proposed in 2021, which catalyzed a 1,200\% increase\footnote{Based on public data for 2021 and 2022 from the AI Index 2024 Annual Report by Stanford University \cite{ai_index_steering_committee_institute_for_human-centered_ai_stanford_university_ai_nodate}.} in regulatory activities in the following year. Such regulatory momentum highlights the Act's global influence and the growing recognition of AI's ethical and societal implications.

While the AI Act lays down provisions for addressing discrimination, its scope should be broadened to include specialized directions targeting economic disparities perpetuated by AI systems. Such disparities are deeply rooted in socio-economic status (SES) that disproportionately impact historically disadvantaged groups~\cite{ganty2021expanding}. For instance, individuals subjected to discrimination based on traditional status grounds, such as gender and race, are often overrepresented among economically disadvantaged populations~\cite{ganty2021poverty}. 
This intersectionality of SES with existing vulnerabilities~\cite{atrey2018intersectional} exacerbates systemic inequities, 
strictly violating the principles of equalization~\cite{dworkin2018equality}, which advocate for equalizing resources or opportunities to mitigate disadvantages beyond an individual's control. 

Despite advancements in AI fairness definition \cite{barocas_fairmlbook, castelnovo2022clarification}, none of the existing notion recognizes the compounded effects of the economic privilege of SES, in generating unfair advantages~\cite{korom2016inherited,morck2000inherited}. Its inclusion in fairness-aware methodologies remains scarce, creating a critical gap in evaluating and mitigating the influence of economic privilege in producing biased outcomes w.r.t. protected features like gender~\cite{kilbourne1997ses_gender}, race~\cite{williams2017wealth,kochhar2014wealth}, etc.
In this work, to address this gap, we propose a novel fairness notion, Socio-Economic Parity (SEP), and a stricter version of it, namely Conditional Socio-Economic Parity (CSEP), that explicitly incorporate SES, advocating for positive actions toward underprivileged groups while accounting for factors within an individual's control, such as working hours, as highlighted in economic principles. 
Using a real-world dataset (Adult~\cite{adult}), we demonstrate that existing popular fairness notions like Equal Opportunity~\cite{hardt2016equality}, Demographic Parity~\cite{dwork2012fairness}, and Conditional Demographic Parity (CDP)~\cite{toon2012book}, fail to recognize SES-driven biases, inadvertently favouring economically privileged groups. To integrating SES into fairness modeling, we define a new fairness measure and optimize a constrained model based on our SEP (and CSEP) notion.

Our empirical results highlight the effectiveness of our approach in both measuring and mitigating SES-driven bias. Furthermore, through an analytical study of the AI Act in parallel with our proposed method, we suggest a foundation for fostering dialogues that align AI fairness with economic and financial applications. This work contributes to bridging the gap between fairness-aware machine learning research and regulatory frameworks, emphasizing the importance of addressing socio-economic disparities in AI systems.


%Henceforth, addressing such socio-economic disparities becomes imperative, which otherwise creates feedback loops that perpetuate privilege for the economically advantaged while marginalizing underprivileged groups~\cite{ganty2021poverty}. 

Unfair treatment and discrimination \cite{hleg2019ethics, information_commissioners_office_ico_guidance_2024} have been widely recognized as major ethical concerns for AI systems \cite{access_now_human_2018, latonero_governing_2018, muller_impact_2020} (commonly termed as AI Bias/ AI unfairness). The increasing global adoption of laws related to AI has become particularly evident in recent years \cite{etchemendy_ai_2024}, while the proposal of the AI Act in 2021 led to a 1.200\% increase\footnote{This calculation was made based on the public data for the years 2021 and 2022, from the AI Index 2024 Annual Report by Stanford University \cite{ai_index_steering_committee_institute_for_human-centered_ai_stanford_university_ai_nodate}.} (in the year following the proposal, namely 2022), further highlighting its significant global influence. Alongside this regulatory momentum, the increasing integration of AI across all facets of society and economic activity attests to its pervasive impact.

While several fairness metrics have emerged in the field of machine learning \cite{barocas_fairmlbook, castelnovo2022clarification}, an essential dimension to consider is their interaction and possible integration with the newly enacted EU AI Act \cite{noauthor_regulation_2024}. On the one hand, the definition and implementation of fairness metrics for addressing AI bias must align with applicable legal frameworks. On the other hand, AI fairness metrics have the potential to initiate discussions about new standards\footnote{On May 22, 2023, the European Commission (EC) issued a standardisation request to CEN and the CENELEC regarding AI Act (Implementing decision C(2023)3215). Available at: https://ec.europa.eu/growth/tools-databases/enorm/mandate/593\_en.}, guidelines, and assessment tools by providing practical solutions.

While there are several critiques \cite{barocas_fairmlbook, wachter2021cdp} of existing AI fairness notions, to the best of our knowledge, none have emphasized the critical role of Socio-Economic Status (SES) \cite{goyder2002SES}. Particularly, the influence of economic privilege in producing biased outcomes~\cite{haneman2021wealth, kochhar2014wealth, korom2016inherited, williams2017wealth, morck2000inherited} has not been thoroughly investigated. SES has been highlighted as requiring increased attention due to its legal protection in discrimination contexts \cite{ganty2021expanding} and its significant implications for AI applications. The importance of addressing the feedback loop of socio-economic precariousness has been recognized \cite{ganty2021poverty}, along with the potential for courts to consider vulnerable groups defined by SES due to structural disadvantages \cite{gerards2022protected}. Despite a growing body of research highlighting the prevalence of SES-based discrimination and the urgent need for its mitigation \cite{atrey2018intersectional, kadar2016analysis, benn2020big, ganty2021expanding, niall_crowley_equality_2015}, this factor has yet to be fully integrated into the EU’s anti-discrimination legal frameworks \cite{ganty2021expanding}.

In this work, using a running example based on real-world data (Adult~\cite{adult}), we first examine the drawbacks of existing popular AI fairness notions and affirm prior findings \cite{wachter2021cdp} that Conditional Demographic Parity (CDP) is among the best approaches. However, we also demonstrate that CDP fails to account for the effects of economic privilege and, therefore, inadvertently promotes bias favouring the economically privileged. Building on this, we propose a new AI fairness notion namely, Socio-Economic Parity (SEP), and a stricter version of it, namely Conditional Socio-Economic Parity (CSEP), which incorporates SES, advocating for positive actions towards the underprivileged, while considering individual-level exerted effort to establish unbiased AI decisions. Based on the notion of SEP (and CSEP), we introduce a new fairness measure and train a constrained model using the conditions defined by it. %our proposed notions SEP and CSEP, and 
We empirically demonstrate its effectiveness in both measuring and mitigating SES-driven bias in AI decisions.




%%%%%%%%%
European Court of Human Rights, Petrov v. Bulgarie, Application
no. 15197/02 (22 May 2008) (as for the marital status);
%%%%%%%%%






%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
We assume a supervised fairness-aware machine learning set-up, where  a dataset (e.g. a census report, marketing data, etc.) $\mathcal{D}$ drawn from an independent and identically distributed (i.i.d.) sample space $\mathcal{P}(X,S,Y)$. The feature space $X$ denotes the collection of unprotected attributes (e.g. professional experience, job, education, etc.), $S$ denotes the collection of protected attributes  (e.g. race, sex, religion, etc.), and $Y$ denotes collection of target class attributes (e.g. loan approval, CV score, salary scale, etc.).  
Traditionally, the attributes of $S$ defines the historically known, and legally acknowledged \cite{fundamental_rights_2007} grounds of discrimination (e.g. demographic groups like females, or subgroups like black females), which needs to be protected when making automated decisions $P(\hat{Y})$ based on feature value distribution of $X$, on learned target distribution defined by $Y$.  
Without loss of generality, for convenience, we consider $Y\in\{0,1\}$ to consist of a single binary attribute  with $Y=1$ as favourable outcome (e.g. granted loan). The idea is easily extensible to a collection of multi-valued multiple attributes. 

Now, using the above set of notations most of the existing fairness definitions can be formalized as follows:
\begin{equation}\label{eq:generic_fair}
\mathbb{E}(h(x)\mid s,C)=\mathbb{E}(h(x)\mid \overline{s},C)), ~~\forall (x,s,y)\in\mathcal{D} 
\end{equation}
where $\mathbb{E}(h(x))$ denotes the expectation of favourable outcome of a predictor $h$ on the non-protected features $x$, $s$ and $\overline{s}$ respectively denotes unprotected and protected %\footnote{throughout the text we use the words underprivileged and protected interchangeably, conveying the same meaning of population against whom historically discrimination is evidenced} 
groups ($s,\overline{s}\in S$) or subgroups ($s,\overline{s}\in S\times S$), and $C$ provides the necessary conditions~\cite{RoyFact23} to define the particular fairness notion. Based on the fairness definitions further, corresponding fairness metrics can be defined using similar generic formulation~\cite{manios2024towards}. 
Now, based on Eq.~\ref{eq:generic_fair}, we explore the different popular fairness notions %that are inspired from some existing legal literature, 
to understand their applicability, the currently prevalent legal and socio-economical concerns that they address, their potential drawbacks, and motivation behind our study. Throughout the exploration we use the popular `Adult' data~\cite{adult} as $\mathcal{D}$ and predictions from a constrained optimization as our $\hat{Y}$, to establish our concrete practical understanding. 


\subsubsection{\textbf{Equal Opportunity (EP)}~\cite{hardt2016equality}:} The formulation given in Eq.~\ref{eq:generic_fair} refers to the fairness notion Equal Opportunity when we have  $C$ as $(Y=1)$, conditioned only on the positive ground truth, i.e. $\mathbb{E}(h(x)\mid s,y=1)=\mathbb{E}(h(x)\mid \overline{s},y=1)$. The idea, motivated by the US report on the call for `\textit{equal opportunity by design}', in general aligns well with the goal of optimal learning, where correctness of predictions across the various demographics is promoted. However, due to various social and historical factors, the datasets used for testing are often biased in class representation among various populations. In Fig.~\ref{fig:run_exp_adult} we see as a running example that a EP-aware classifier~\cite{agarwal2018} which has learned to produce (nearly) perfect predictions with high True Positive Rates (TPR) $P(h(X)=1\mid Y=1)$ and low False Positive Rates (FPR) $P(h(X)=1\mid Y=0)$ for both males and females, has still a high difference in Positive Prediction Rates (PPR) $P(h(X)=1)$. This outcome is due to the demographically specific ground truth (class) imbalance, as the probability of favourable outcomes within the females ($P(Y=1|S=`females')$) is much lower than that of males in the Adult dataset.  An extreme example of the problem reported by Roy et al.~\cite{RoyFact23}, shows that `black young females' have probability of $\small \frac{1}{61}\normalsize$, whereas `white old males' have probability of $\small \frac{1}{1.6}\normalsize$ for favourable outcome in the Adult data. This imbalance problem is not unique to the Adult data, and is seen in most of (if not all) the dataset used in fairness-aware learning~\cite{tai2022survey}. Such variation in class distribution reflects existing inequality and injustice captured within the ground truth, and preserving EP in this case further promotes the societal imbalance~\cite{barocas_fairmlbook}.  
% The problem holds true even for the stronger `Equalized Odds'~\cite{hardt2016equality} (EO) definition, where the requirement for $C$ is conditioned on both the classes, i.e., $(y\in\{0,1\})$, to hold equality in false positive along with true positives. Note that the EP-aware classifier also have (almost) equally low FPRs for males and females. 

\subsubsection{\textbf{Demographic Parity (DP)~\cite{dwork2012fairness}:}}
In Eq.~\ref{eq:generic_fair} when the expected outcome of $h$ is free from any dependency i.e., $\mathbb{E}(h(x)\mid s)=\mathbb{E}(h(x)\mid \overline{s})$, we obtain the definition of Demographic Parity (DP). The idea is motivated from the discrimination against racial protected population in the financial domain where a credit card company was guiding members of protected groups into less advantageous credit offerings ~\cite{wallstreet2010}. To understand its applicability, we refer to  Fig.~\ref{fig:run_exp_adult}, which shows that when a fairness-aware classifier is trained with DP constraints~\cite{agarwal2018}, it produces predictions with nearly equal Positive Prediction (PP) rates for males and females. It achieves so by predicting higher false positives for females. Allowance of such selective error may be justified as `Affirmative action'~\cite{affirmative_anti_discri2011} as it apparently addresses the previously observed imbalance injustice. However, researchers has often expressed their concerns regarding the negative impact of such unconditional promotion, potentially increasing the existing negative prejudice against the protected groups (e.g., by selecting higher number of unqualified candidates)~\cite{barocas_fairmlbook}. To understand the impact better, we look into per `occupation' class distribution of females and males. For reference, first we look at the ground truth distribution of males and females per occupation in Fig.~\ref{fig:dist_by_ocu_true}. We readily notice the extreme under-representation of the positive female labels across all the occupation. Henceforth, simply training an highly accurate model to mimic the ground truth distribution or to match the overall positive prediction rate won't resolve the imbalance problem and would further widen the positive class representation between different demographics in certain occupations.  This practical impact is well established in Fig.~\ref{fig:dist_by_ocu} where
comparing the predictions by the EP-aware and the  DP-aware classifier we notice that both EP-aware and DP-aware classifier predicts males with certain occupation like `Executive managerial' and `Professional speciality' are expected to earn high (more positive `>50K' than negative `$\leq$50K' class labels). However, for females working in these professions, neither the predictions from the EP-aware, nor from the DP-aware classifier narrates a similar storyline.   

\subsubsection{\textbf{Conditional Demographic Parity (CDP)~\cite{toon2012book}:}} Stated in the literature as gold standard~\cite{wachter2021fairness},  conditional demographic parity (CDP) extends the demographic parity notion with an additional condition on an (usually a categorical unprotected) attribute (say $X_a$). The requirement to observe equality in PPR between the non-protected and protected, for all categories in the selected conditional feature (i.e., $\forall a \in X_a$). Formally, we can define CDP using Eq.~\ref{eq:generic_fair} as $\mathbb{E}(h(x)\mid s,a)=\mathbb{E}(h(x)\mid \overline{s},a)),~~\forall a\in X_a$. The idea is motivated from the study of `\emph{Redlining}'~\cite{rice1996redlining} effect which affected protected racial demographic from getting equability of access to financial services such as bank loans based on proxy attribute such as location. To understand its applicability we look to the prediction from a CDP-aware classifier on our running example. We trained this model with the attribute `occupation' as our conditional feature $x_i$.  
In Fig.~\ref{fig:run_exp_adult} we notice that the CDP-aware classifier almost matches the DP-aware classifier in producing nearly equal PPR for males (0.28) and females (0.24) while maintaining high TPRs (>0.86). But,  in Fig.~\ref{fig:dist_by_ocu} we see a stark difference, with CDP-aware classifier being able to  match the rate of positive predictions for females and males across all the occupations. It overcomes the previously observed drawbacks of EP-aware and DP-aware classifiers by predicting higher expectancy of high income than low income  by females in the high income professions (`Executive managerial' and `Professional speciality') for males. 

\subsubsection{\textbf{Should CDP be the gold standard of fairness in socio-economical context?}}\label{sec.cdp_gold}
From Fig~\ref{fig:dist_by_ocu} we know that the CDP-aware classifier is certainly a better notion than DP and EP in positively promoting females (protected demographic). However, it is still not clear on what factors the model relied upon while making the so-called fair outcomes. 
Studies have shown that possession of inherited large wealth~\cite{korom2016inherited,morck2000inherited} has been a source of economic privilege in influencing opportunities~\cite{haneman2021wealth}, often rooting to societal bias~\cite{kochhar2014wealth,williams2017wealth}. Although the \emph{Adult dataset} used in our running example, does not include a feature explicitly representing wealth or asset privilege, it does contain a \texttt{capital-gain} feature, which can serve as a proxy for wealth~\cite{Mitchell2023reportCapitalGain}. 
Interestingly, capital gain in the Adult data has often been found in studies~\cite{panagiotou2024tabcf} to bore a strongly positive impact on the predicted outcome.  

To examine the influence better, we subdivide the data into groups of `Privileged' (with 5\% capital gain among all individuals), and `Underprivileged' (rest of the 95\% individuals) based on the feature \texttt{capital-gain}. In this way, we get four subgroups, namely `privileged males', `privileged females', `underprivileged males', and `underprivileged females'. We plot the predicted outcomes of the CDP-aware classifier on our identified subgroups in Fig~\ref{fig:work_hour}. We notice that for the privileged groups the CDP-aware classifier provides highly favourable outcomes, with positive prediction rates (PPR) of 90.15\%  for privileged males (ground truth is 91.88\%), and 86.33\% for privileged females (ground truth is 81.77\%). Even though there exists a gap in performance between the two privileged subgroups,  this outcome is still comparable adhering to the 80\% rule~\cite{dwork2012fairness}, mainly owing to the fair distribution of the positive labels in the ground truth for the privileged. For the underprivileged groups, however, the PPR falls sharply to 23.73\% (74\%$\downarrow$) for males, and to 21.87\% (75\%$\downarrow$) for females. This biased outcome shows the clear impact of socio-economic privilege in garnering favourable outcome. However, it is still a fairer outcome when compared with the ground truth, which contains only 9\% underprivileged females, whereas 27\% of underprivileged males are labelled as positive. Clearly, a lot of false positives for entire female demographic comes from the underprivileged females (almost 99\%), which can be argued as necessary in order to promote affirmative/ positive actions. 

A question may arise concerning the merit of the underprivileged females that are promoted to the positive class (false positives), i.e. are they the best/most deserving candidates? Promotion of more undeserving candidates is criticised to have the ability to increase negative track record and henceforth negative sentiment towards the protected demographics~\cite{barocas_fairmlbook}. Selection of deserving candidates can again be the subject of debate. However, economic literatures~\cite{cappelen2009rewarding} often argue that positive actions (reward) to individuals should be based on factors under the control of individuals (e.g., physical or mental efforts) to establish the principle of equalization~\cite{dworkin2018equality}. For the Adult data, among the set of available features, we use working \texttt{hours-per-week} (matches with the argument of factors under the control of individuals) as the measure of individual effort put in a respective job~\cite{becker1985effort}. Now, for the sake of argument, we identify individuals working more than the mean working hours as individuals with high effort, and again refer to the performance of the CDP-aware classifier depicted in Fig~\ref{fig:work_hour}. We observe that PPR of the model on both the high effort subgroups (34.27\% for females and 36.72\% for males) is better compared to the overall underprivileged subgroups. However, a closer analysis reveals that the FPR is only 20\% which is just 21\% of all the false positive made for all the underprivileged females, and ironically is lesser than the FPR (25\%) for privileged females.    

In summary, our observation reveals that protected groups when have access to privilege generates a favourable chance nearly equal to that of privileged non-protected. We argue that underprivileged individuals who can be considered as putting in high effort deserves a fair chance  getting a favourable outcome when compared with subgroup of Privileged individuals, in order to minimise the effect of wealth disparity. Following the theory of equalization~\cite{dworkin2018equality}, such positive reward should ideally be weighted based on the evaluated effort by the individual. Moreover, for privileged subgroups, the ground truth rate of favourable outcome is high, henceforth, positive action towards such subgroup can be considered as under utilization of available resources.  
The CDP notion fails to capture the explicit disparity of wealth in the socio-economic context, and has no explicit mechanism to positively reward the needy and deserving candidates. Henceforth, the CDP-aware classifier in our example, conditioned upon producing equal PPR w.r.t., the attribute `occupation', does not learn to reward the candidates who does not have the economic privilege of capital gain, but within their respective population puts relatively higher effort. %and have the  best possible access (within community) to favourable outcome.  


Figure~\ref{fig.positive_action_comparison} further compares PPR rates by hours-per-week for  underprivileged males and females under EP-, DP-, CDP-, and CSEP-aware models. Notably, CSEP allocates positive outcomes to high-effort underprivileged females (here $\geq$ mean effort), almost doubling the female/male PPR ratio (0.98 to 2.1), helping to mitigate both overall demographic disparities and those affecting protected underprivileged subgroups observed in the ground truth (Fig.~\ref{fig:dist_by_ocu_true}). In contrast, EP- and DP-based methods under-reward these high-effort females, resulting in lower PPRs than their male counterparts. The CDP-aware although distributes higher PPR to all the underprivileged but distributes it equally between both the demographics, henceforth failing to foresee required positive action required to promote more deserving underprivileged females to tackle the overall disparities between the two. 

Figure~\ref{fig.positive_action_comparison} further compares PPR rates by hours per week for underprivileged males and females under EP-, DP-, CDP-, and CSEP-aware models. Notably, CSEP allocates positive outcomes proportionally to effort among high-effort underprivileged females ($\geq$ mean effort), nearly doubling the female-to-male PPR ratio (0.98 to 2.1) and mitigating both overall demographic disparities and those observed among protected underprivileged subgroups (Fig.~\ref{fig:dist_by_ocu_true}). Specifically, the PPR for underprivileged females increases from below 0.3 for those working fewer than the mean hours to above 0.6 for those exceeding it, reaching nearly 0.7 for those working 55 hours or more. In contrast, EP- and DP-based methods under-reward these high-effort females, resulting in lower PPRs than their male counterparts. Although the CDP-aware model provides higher PPR for all underprivileged individuals, it does so uniformly across both demographics, failing to deliver the additional positive actions needed to support high-effort underprivileged females and address remaining disparities.


%%%%%%%%%%%%Conclusion

In this work, we introduced Socio-economic Parity (SEP), a novel fairness notion supported by a corresponding fairness measure, and we provided legal perspectives under the EU framework regarding discrimination in AI. This interdisciplinary approach fosters the convergence of legal studies and machine learning in several key domains:

\noindent\textbf{A foundation to prevent financial exclusion by examining privileged and unprivileged groups.} 
The success of SEP arises from verifiable, transparent model outputs that are backed by comprehensive legal justifications. The introduction of comparators’ groups via indirect discrimination serves as a valuable mechanism for identifying and correcting inequities between privileged and unprivileged SES-based subgroups.
